On the Iteration Complexity of Smoothed Proximal ALM for Nonconvex Optimization Problem with Convex Constraints

It is well-known that the lower bound of iteration complexity for solving nonconvex unconstrained optimization problems is $\Omega(1/\epsilon^2)$, which can be achieved by standard gradient descent algorithm when the objective function is smooth. This lower bound still holds for nonconvex constrained problems, while it is still unknown whether a first-order method can achieve this lower bound. In this paper, we show that a simple single-loop first-order algorithm called smoothed proximal augmented Lagrangian method (ALM) can achieve such iteration complexity lower bound. The key technical contribution is a strong local error bound for a general convex constrained problem, which is of independent interest.

==> SProxALM [SIAMOPT] (Submit, axriv)/ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.

%%%%%%%%%%%%%%%% Wenqiang %%%%%%%%%%%%%%%%%%%%%%
\usepackage{enumerate}
\usepackage{enumitem}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{latexsym,bm,amsfonts}%amsfonts

\newtheorem{thm}{Theorem}
\newtheorem{lem}{Lemma}
\newtheorem{prop}{Proposition}
\newtheorem{coro}{Corollary}
\newtheorem{rmk}{Remark}
\newtheorem{defi}{Definition}
\newtheorem{asp}{Assumption}
%%%%%%%%%%%%%%%% Wenqiang %%%%%%%%%%%%%%%%%%%%%%

% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\usepackage{hyperref}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{ }{J. Zhang, W. Pu, and Z.-Q. Luo.}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{On the Iteration Complexity of Smoothed Proximal ALM for Nonconvex Optimization Problem with Convex Constraints\thanks{Submitted to the editors DATE. Jiawei Zhang and Wenqiang Pu contributed equally.
\funding{The work of Wenqiang Pu is supported by the National Natural Science Foundation of China (No. 62101350). The work of Zhi-Quan Luo is supported by the National Natural Science Foundation of China (No. 61731018) and the Guangdong Provincial Key Laboratory of Big Data Computing.}}}

% Authors: full names plus addresses.
\author{Jiawei Zhang$^\ddagger$\thanks{Laboratory for Information and  Decision Systems, Massachusetts Institute of Technology, USA
  (\email{jwzhang@mit.edu}).}
\and Wenqiang Pu\thanks{Shenzhen Research Institute of Big Data, The Chinese University of Hong Kong, Shenzhen, China 
  (\email{wenqiangpu@cuhk.edu.cn}, \email{luozq@cuhk.edu.cn}).}
\and Zhi-Quan Luo\footnotemark[3]}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

